A Game-Based Approach for Helping Designers Learn Machine Learning Concepts

Machine Learning (ML) is becoming more prevalent in the systems we use daily. Yet designers of these systems are under-equipped to design with these technologies. Recently, interactive visualizations have been used to present ML concepts to non-experts. However, little research exists evaluating how designers build an understanding of ML in these environments or how to instead design interfaces that guide their learning. In a user study (n=21), we observe how designers interact with our interactive visualizer, \textit{QUBE}, focusing on visualizing Q-Learning through a game metaphor. We analyze how designers approach interactive visualizations and game metaphors to form an understanding of ML concepts and the challenges they face along the way. We found the interactive visualization significantly improved participants' high-level understanding of ML concepts. However, it did not support their ability to design with these concepts. We present themes on the challenges our participants faced when learning an ML concept and their self-guided learning behaviors. Our findings suggest design recommendations for supporting an understanding of ML concepts through guided learning interfaces and game metaphors.

==> notes/CHI2020_edits.tex <==
EDITS
* Describe how QUBE works in more detail
* Fix image of QUBE with Labels and boxes
* Look into theme table and how that analysis works
* Crystalize how people interact with this system
* Incorporate Jichen's Results edits
* Incorporate Jichen's Discussion edits
* Layout images and pages
* Check the references
* Remove Q-Learning Def of ML
* More details in Right Way
* Look into more insights like parameter manipulation
* Remove QUBE tut slides
* Keep example GANLab Tensorflow but screen shot highlight the unstuctured exploration based learning. If it DOESN'T highlight then don't include. 
* Include time limit into study design.
* Report how many people decided not to interactive with the reinforcement agent.
* How do people choose to use this agent shows their mental model. How can we tell what these designers, how they are inclined to interact? Strengthen gradual complexity. 
* more evidence for simple to complex
* simple to complex, easier factors on top. Organize for experimentation
* tie arbitrary parameter values to tensorlfow
* isolate how our tool is similar to tensorflow and ganlab
* add quote about range of parameter values


---------------------------

DONE




---------------------------

OVERALL

The more we summarize how people interact with it the stronger it can be. WHAT THEY DID > WHY THEY DID IT

Simple to complex > how visible in it in interface and affect. Give concrete examples what they did. Behavior patterns. More interesting things provided here. 

What informed concrete decision for what to play with first. 

Preselected subset of parameter values

This is not us just evaluating QUBE. Here is what is in common to Tensforflow and GANLab. 
- subset of parameter values
- sandbox for exploratory playground
- simulation-based interactive visualization

Priority -> Findings.
Structure findings about things that are common in similar system. Game specific 

What are the goals of the participants when interacting with this tool? 

+alternative approaches where BLANK


==> notes/UIST2020_DiscussionOutline.tex <==

Overall
- We keep seeing new IV being made but we have shown that these only support a high level understanding.
- Recent research shows that designers are capable of achieving this high-level understanding outside of IVs (Yang, Dove), so why are we building systems that still only scratch the surface of ML education.
-We present design recommendations for guided learning experience for RL and ML when generalizable. 



Parameter Relationships
- We designed mad libs based on XAI Lime and NLP to highlight the impact of the the understanding of each parameter. This worked. There was a high-level understanding of each parameter but this was not enough to support achieving design goals. Because while this defined what each parameter did, it does not address #1) the severity of the impact and #2) the impact on other parameters. - This is applicable to all ML concepts with changable parameters.
- XAI and IML will play an important role in designing education systems for ML concepts. There are a lot of techniques to choose from, how do we select which ones to incorporate into our system? Future educational systems should explore XAI techniques that focus on these two features, severity and relationship. 
- Severity can be represented to the user by what is the predicted impact of their change. Teachable machine includes this in a tooltip for learning rate. Information the users a small change will make a big impact. We believe that is parameter's values were abstracted in high/low values, that this range could also highlight the severity of the change. Color could be used to show a slight change could have a big impact.
- Relationship Cheng 2016
- Instead of our approach which teaches individual parameters, highlight the relationship

==> notes/discussions.tex <==
%--------------------------------------------
% DISCUSSION
%--------------------------------------------
\section{Discussion}
% - Meaning of values, abstract (low to high). Explain or reduce. 
% We believe our findings on behavior in a sandbox environment, interaction with simulation IV, and manipulation of parameters are generalizable to other IV with these characteristics targeting designers. These characteristics are also not unique to RL. Our findings on our mad-lib explainers and game domain are, however, unique to IVs seeking to also incorporate these features.

Overall, \textit{QUBE} was found to statistically significantly improve our participants' definitions for ML and Q-Learning. Our thematic findings highlight several behavior patterns of designers exploring RL concepts in an IV. In general, the IV of Q-Learning greatly aided our participants in interpreting the algorithm. Our analysis on how participants interacted in \textit{QUBE's} sandbox environment, IV simulation, manipulable parameter, and features unique to \textit{QUBE} (e.g., mad-lib explainers) led to design implications for designing IVs presenting ML concepts for designers.  

%Next, we present design implications for uses metaphors, supporting exploration, understanding the ML process, and designing parameters.



\subsection{The Effects of Metaphors}
%discuss
Participants appreciated learning through metaphors and they made the concepts presented more approachable. However, as these RL concepts were abstracted to a game domain, the abstraction fostered implicit goals characteristic of the domain. We observed participants assume the ``best'' or ``right'' way to design the agent was to make it as fast as possible in solving the maze. We speculate this belief was fostered by the game-like nature of \textit{QUBE}. Since the maze is a game it comes with competitive characteristics. Mazes are puzzles meant to be solved and competition could influence a user to want to solve it quickly. Since IVs are sandbox environments with no explicit goals, participants relied on these implicit goals to structure their exploration. These implicit goals could be leveraged purposefully to guide designers exploring IVs for ML concepts. The domains and metaphor can be chosen to match the desired goals of the IV's designer. For example, if we wanted to guide designers to design for exploration rather than speed with Q-Learning, we could have \textit{QUBE's} agent play ``hide-and-seek'' instead of completing a maze. Players of ``hide-and-seek'' value thorough exploration over speed. Additionally, presenting Q-Learning parameters in a single game domain did limit participants ability to generalize outside the domain. By selecting the ``reward'' and ``punishment'' metaphor, participants felt punishment was a harsh consequence for the anthropomorphized agent and valued rewarding the agent more. Future IVs for ML concepts should evaluate how their selected domain limits designers' generalization of the concepts presented to other domains and affects designers' approach to customizing parameters.  

We encourage future researchers to consider the implicit goals their selected domain or illustrative metaphors may create. We suggest that when choosing metaphors or a domain for ML education to additionally apply the concept outside of the metaphorical boundaries. To combat this, instead of selecting one domain (e.g., maze design), an IV can present ML concepts in various domains. We recommend presenting interactive examples to demonstrate various applications instead of relying on text and tutorials since participants responded positively to the IVs helping them understand the underlying concept.  


% Alternatively, the domain can be carefully select so the implicit goals align with the goals of the IV as discussed.  

% . This lead to several users misinterpreting color or giving color more meaning than it had. Researchers of future ML education tools for designers should pay close attention to color choices and the meaning they can convey.  











% \textit{``Because the explanation that's given tells you what effect it has. So if my goal coming into this, is to make it, make the agent learn the path as quickly as possible, then I just want to set the parameters to do that. So I didn't really feel a need to change them from what I was told would make the agent learn the fastest.''} [P7]

% Additionally, we observed participants apply human traits to entities in \textit{QUBE}. Presenting Q-Learning through ``reward'' and ``punishment'' examples influences our participants selection for these values.

% By selecting a maze domain, we presented our designers with the assumed goal ``fast'' was best. By selecting the ``reward'' and ``punishment'' metaphor, we presented the assumed goal of ``punishment'' being a harsh consequence.

% Lastly, for any user the importance of design is obvious. For our non-experts, the design of \textit{QUBE} was especially crucial since non-experts do not have the formal RL education to fall back to understand the presented concepts. Instead, designers were observed to fall back to their understanding of color and media (e.g., video games)



%design





% We also suggest to demonstrate where a ML example resides in the hierarchy of ML and ML-subsets if presenting concepts through an single ML example. In the tutorial, we do explain that Q-Learning is a subset of Reinforcement Learning (which is a subset of ML). We also discuss unsupervised and supervised learning. P11 points out she is confused on their relationship. \textit{``Confused how this relates to supervised learning, unsupervised - 'I'm like, would they be the same thing? Like maybe you play through the level a couple times and then let the AI try and figure that out? based off of what you've done?' I don't know. I don't code.''} By providing contrasting examples, designers can be given a broader picture on what is ML and its applications. P18 believed she understood less about ML by using \textit{QUBE} because it demonstrated ML to be a bigger field than imagined. \textit{``I am having trouble answering this questions because I know what I put before. And I feel like I know less because the breadth of what I was shown is deeper.''} By provided a ML ``roadmap'' non-experts can contextualized what they are learning and see scaffolding to explore more ML concepts.








% However, the purpose of our analysis was not to support or reject sandbox IVs but instead to observe how designers structure their own interaction.
% As discussed, complexity was determined by visibility.
% Our designers also expressed different goals when exploring \textit{QUBE}. We do not generalize the goals of challenging the agent and speed to other ML concepts since we speculate these goals were influenced by \textit{QUBE's} game domain.

% The goal of experimentation was a common approach our participants took to exploring \textit{QUBE}. While we speculate specific examples can help participants isolate the effect of ML concepts, designers can be supported to design their own experiments as well. Designers need to be able to compare the results of the experiments with tool such as our snapshot tool. We found the natural language in our mad-lib explainers assisted our designers in designing their maze and experiments. 




%design


% Researchers designs IV can conducted usability tests such as our to identify self-defined goals and take steps to support or correct them. 

%  Future IVs can assist designers with their experimentation by embedding more natural language descriptions explaining parameters.








\subsection{Understanding the RL Process}
%dicuss
IVs attempt to make the underlying process of its algorithm transparent through simulation. However, our participants were confused by the their role in this process and the amount of data the agent was considering while solving the maze. Participants were unsure of what their responsibilities were when the agent was cycling through the maze. In \textit{QUBE} and \textit{TensorFlow Playground}, the IV does not show an end state for users to compare their progress. Our participants were confused when watching the agent cycle since it was not clear what the agent was working towards or what the users should be doing at that time. Additionally, it was not clear to what data the agent was considering and when to reset these considerations. \textit{TensorFlow Playground} handles this issue by automatically resetting training. However, editing some parameters resets training automatically while others do not. Based on our findings, we speculate this inconsistency can further confuse designers.

To address this, ML IVs can share example end states of the simulation for designers to compare their progress. Automatically resetting training data can reduce the issues observed by participants forgetting to do this step. We suggest this automation be made transparent as well so the ML process is not lost to the designer and the necessity of resetting missed. 




%design
 

% Another approach in making the ML process transparent is by automating it. In the example of participants forgetting to reset after training, this reset could be done automatically for them if they make any change to the maze design.   

% Our designers often lacked the meta-knowledge to structure their exploration effectively. Yet, the ability to interact with the visualization process provided designers the ability to still isolate the effect of maze design features and parameters which, in turn, helped their understanding.


\subsection{Designing Parameters for Interaction}
%discuss
Finally, it may make sense to a ML expert the difference between a learning rate of 0.5 to 1 but this is not transparent to designers. The logic behind the increments and the range selected is not easily interpretable. We believe that abstracting the values even further would be more beneficial.




%design
One solution could be to explain the range and increments to the designer.  Instead of selecting a goal reward of 1 to 100, we could allow designers to select on a value on an abstract scale of ``low'' to ``high.'' 

Additionally, participants were confused on how parameters effected each other. Researchers can assist in this understanding by creating experiments for designers to explore demonstrating the effect parameters have on each other (an approach mentioned in the previous section).


Researchers can also include this in the descriptions of the parameters (e.g., goal reward and punishment value can be presented together to illustrate their relationship). A third option could be to relate parameters to the self-defined goals of the designers. We can tell designers what parameters of Q-Learning help or harm these goals. For example, \textit{QUBE} can be augmented with a sidebar providing tips on how to reach these goals. For challenging the agent, a high range of movement of the ghost and high punishment value will made the maze more difficult. These tips also have the potential to help designers structure their own experiments. 













